MobileDets: Searching for Object Detection Architectures for Mobile Accelerators

Inverted bottleneck layers, which are built upon depthwise convolutions, have been the predominant building blocks in state-of-the-art object detection models on mobile devices. In this work, we investigate the optimality of this design pattern over a broad range of mobile accelerators by revisiting the usefulness of regular convolutions. We discover that regular convolutions are a potent component to boost the latency-accuracy trade-off for object detection on accelerators, provided that they are placed strategically in the network via neural architecture search. By incorporating regular convolutions in the search space and directly optimizing the network architectures for object detection, we obtain a family of object detection models, MobileDets, that achieve state-of-the-art results across mobile accelerators. On the COCO object detection task, MobileDets outperform MobileNetV3+SSDLite by 1.7 mAP at comparable mobile CPU inference latencies. MobileDets also outperform MobileNetV2+SSDLite by 1.9 mAP on mobile CPUs, 3.7 mAP on Google EdgeTPU, 3.4 mAP on Qualcomm Hexagon DSP and 2.7 mAP on Nvidia Jetson GPU without increasing latency. Moreover, MobileDets are comparable with the state-of-the-art MnasFPN on mobile CPUs even without using the feature pyramid, and achieve better mAP scores on both EdgeTPUs and DSPs with up to 2x speedup. Code and models are available in the TensorFlow Object Detection API: https://github.com/tensorflow/models/tree/master/research/object_detection.

==> previous-reviews.tex <==
\subsection{Updates and Resubmission Rationale}
A key contribution of our submission is the development of new NAS search spaces and models that specifically target hardware accelerators for mobile phones, such as DSPs, EdgeTPUs and edge GPUs. In contrast, most previous NAS research either (i) explicitly optimized for FLOPS or CPU latencies, or (ii) reused search space primitives such as inverted bottlenecks which were originally developed for CPUs. In this work we quantitatively reveal that this limited search space design can be a substantial bottleneck of the performance of NAS for modern mobile accelerators.

However, we believe the above was not communicated well enough in a previous version of our manuscript. For example, R1 from our ECCV submission raised concerns that our models had high FLOPS counts, while R3 and R4 expressed concerns that the paper showed limited performance improvements on CPU.

In addition, the ECCV reviewers were concerned about the novelty of the NAS method (TuNAS) and/or task (object detection), which was the main reason for rejection. These, however, were not the key points which we intended to focus on. In this 6-page submission, we have substantially improved the clarity of the paper to better reflect our main contributions:

New search space family. We propose a new search space family which can substantially boost the performance of NAS methods across a variety of modern mobile accelerators. This is achieved by revisiting full (instead of depthwise) convolutions, which are underexplored in existing mobile NAS works.
State-of-the-art models. We deliver a set of lightweight, easy-to-deploy mobile object detection with state-of-the-art quality-latency trade-offs across EdgeTPUs, DSPs, as well as edge GPUs (new results). Models will be released to benefit a wide range of on-device object detection applications.

Besides improved writing, we also provide new results to demonstrate that our search space design is not only performant for CPUs, EdgeTPUs and DSPs, but can also generalize well to a new hardware platform (Nvidia Jetson GPU).

\subsection{Original Reviews}
\subsubsection{Meta Reviewer}
Comment: After taking the rebuttal into account and reading each others reviews, there is a consensus among reviewers that while the paper is focused on an important topic and some of the reviewers comments were addressed in the rebuttal, the main limitations remain and the novelty and contribution is not sufficient to warrant acceptance at ECCV 2020.  

\subsubsection{Reviewer \#1}
Summary Of Contributions: This paper proposes a NAS method that generates a latency-efficient backbone for object detection. The authors aim to multiple target platforms to reduce the inference speed of a backbone by searching with Inverted Bottleneck, Bottleneck, and their fused block. Experiments are done to support the authors' claim,
Strengths: +) The proposed idea of fusing full-convolution into IB is interesting.
+) Restricting search space looks good.
Weaknesses: -) The novelty is limited. Since the proposed method focuses on finding the backbone for the following detection module SSDLite, there has been a lot of NAS methods that successfully find a classification backbone such as ProxylessNAS targetted to diverse platforms.
-) No comparison with other backbones + SSDLite. For example, MNasNet + SSD-lite (not using NAS-FPN head) can be easily evaluated in Table 1.
-) Limited performance improvement (especially in CPU)
-) The architecture found by the proposed method has large FLOPs and parameters compared to the baselines.
-) The authors constrained the search spaces but the method has still a costly training budget of using 4x4 TPU-v2.

Suggestion To Authors: 1. Why the searched models targetted to DSP show better performance than that of EdgeTPU in the transferability test in Fig 9 (b)? Readers may speculate the searched models would not be close to optimal.
2. A shallow search space could be a benefit to quickly get a model but sometimes looks too restricted. Is there any intuition why the searching space is restricted to block-level? TuNAS looks available to run with operation-level search space.
3. How many TPU (or GPU) times searching for architecture? 
4. Please specify the latency of MobileNetV3 in EdgeTPU and DSP in Table 1.
5. Does the search space include the strides of a convolution layer?
6. SSD-lite mainly uses depthwise convolutions which are not efficient in some platforms such as GPU. Therefore, it is natural to extend the proposed method by considering SSD-lite as well into the search space. 

Preliminary Rating: 3: Borderline reject
Preliminary Rating Justification: Searching for a network architecture for SSD-lite detector may be necessary for a fast object detection task. However, the novelty is limited compared to the previous NAS methods, because the method just finds a backbone and use SSD-lite as a detection head. Furthermore, I don't think this method can be easily adopted because the training time is too costly.


\subsubsection{Reviewer \#4}
Summary Of Contributions: The paper proposes to search a lightweight detection network for mobile accelerators by using regular convolutions, instead of just following the inverted bottlenecks (IBN) in MobileNet v3. All the modifications focus on replacing the depthwise convolution with regular convolution, and have achieved certain results.
Strengths: The motivation is intuitive, and it has important practical value to search lightweight detection network for Mobile devices. The experiments shows the effectiveness on some specific devices.
Weaknesses: 1. Insufficient contributions. The authors should refine and reorganize the contributions, especially in the section of introduction. Moreover, the depthwise convolution will increase the Memory Access Cost (MAC), thus it does not necessarily reduce the inference time. This idea has be demonstrated in ShuffleNet v2 [1], so using regular convolution to replace the depthwise convolution is not that significant.
2. In Fig. 5, the proposed search space (i.e., IBN+Fused and IBN+Fused+Tucker) has no advantages over IBN both in speed and accuracy, the authors should better clarify this.
3. There are no comparisons with the original MnasFPN.
4. The manuscript should be refined carefully, there are many typos and poor sentences.

[1] Ma N, Zhang X, Zheng H T, et al. Shufflenet v2: Practical guidelines for efficient cnn architecture design, ECCV2018: 116-131.

Suggestion To Authors: Some typos and poor expressions: 
Line 34: a lot of effort….
Line 113: most performant models…
Line 248: modulo non-linearities
Line 251: modulo nonlinearities

Preliminary Rating: 3: Borderline reject
Preliminary Rating Justification: Although the paper has achieved certain progresses, the contributions are insufficient, please see the weaknesses.
The paper should be reorganized to highlight the innovations and enhance the readability.

Confidence: 4: High, published similar work
Final Rating: 3: Borderline reject
Final Rating Justification: The authors provide some explanations for my previous concerns. However, I think the main weaknesses still exist, I thus keep my rating unchanged.


\subsubsection{Reviewer \#3}
Summary Of Contributions: (1) This paper searches network backbones targeted for object detection on some specific harewares.  MobileDets, the searched a family of models, achieve surprising results on different hardware platforms.

(2) A new search space --- TDB is proposed by adding two new kind of cell structures ( regular convolution based) into IBNs search space.
Strengths: (1) The searched models --- MobileDets show surprising results on different hareware platforms. 

      For COCO, MobileDets outperform MobileNetV3+SSDLite by 1.7 mAP at comparable mobile CPU inference latencies. MobileDets also outperform MobileNetV2+SSDLite by 1.9 mAP on mobile CPUs, 3.7 mAP on EdgeTPUs and 3.4 mAP on DSPs while running equally fast. Moreover, MobileDets are comparable with the state-of-the-art MnasFPN on mobile CPUs even without using the feature pyramid, and achieve better mAP scores on both EdgeTPUs and DSPs with up to 2x speedup.
Weaknesses: (1) The novelty is limited. 

      I.  Searching for architectures targeted at specific platforms has already been proposed many times, like [4, 30].  

      II. The proposed TDB search space is obtained by only adding ResNet-like cell structure and MLPConv( Network In Network )-like cell structure.
           The connections between ResNet cell structure, Inverted bottleneck sturcture and Tucker/CP decomposition have already been demonstrated by previous works shown below.


 Min Lin et al. "Network In Network". ICLR 2014.
 Chen Yunpeng et al. "Sharing Residual Units Through Collective Tensor Factorization in Deep Neural Networks". IJCAI-18.
 Marcella Astrid et al. "CP-decomposition with Tensor Power Method for Convolutional Neural Networks Compression". 
 BigComp 2017. 


      III. The adopted NAS method has no differences between previous NAS method (TuNAS).
    
(2) What most interested me is the searched model. However, I mainly concerns whether the experimental setting is fair between the searched models and the baselines (MobileNetV2, MobileNetV3).  



Suggestion To Authors: (1) Show the key novelty of the proposed method.

(2) Make sure the experimental setting is fair between the searched model and baselines (MobileNetV2, MobileNetV3), e.g. the training time. The training time has great effects on two-stage object detection frameworks, like Mask-RCNN.
Preliminary Rating: 3: Borderline reject
Preliminary Rating Justification: The paper searches architectures for object detection on different platforms. The searched architectures --- MobileDets show surprising results. 

However, the novelty is limited. Platform aware NAS has been explored by many previous papers. 

The proposed TDB search space is obtained by only adding ResNet-like cell structure and MLPConv-like cell structure. And the connections between ResNet cell structure, inverted bottleneck structure and tensor decompostions have already been demonstrated by previous works.
Confidence: 4: High, published similar work
Final Rating: 3: Borderline reject
Final Rating Justification: I read the other reviews and the author responses. I still hold that the novellty is limited. This paper only apply the NAS to search backbone for detection. I will never change my opinion.


